Dr. Summarize: Global Summarization of Medical Dialogue by Exploiting Local Structures

Understanding a medical conversation between a patient and a physician poses a unique natural language understanding challenge since it combines elements of standard open ended conversation with very domain specific elements that require expertise and medical knowledge. Summarization of medical conversations is a particularly important aspect of medical conversation understanding since it addresses a very real need in medical practice: capturing the most important aspects of a medical encounter so that they can be used for medical decision making and subsequent follow ups. In this paper we present a novel approach to medical conversation summarization that leverages the unique and independent local structures created when gathering a patient's medical history. Our approach is a variation of the pointer generator network where we introduce a penalty on the generator distribution, and we explicitly model negations. The model also captures important properties of medical conversations such as medical knowledge coming from standardized medical ontologies better than when those concepts are introduced explicitly. Through evaluation by doctors, we show that our approach is preferred on twice the number of summaries to the baseline pointer generator model and captures most or all of the information in 80% of the conversations making it a realistic alternative to costly manual summarization by medical experts.

==> sections/3mixturecomparison.tex <==







==> sections/exp.old.tex <==


\section{Dataset}

\TODO{We collected a dialogue dataset using X number of conversations from the Curai Health platform.}  We split up the dialogue into a series of local dialogue (snippets) turns using .. heuristic. doctors who usually summarize the entire dialogue into clinical notes during normal patient encounters were asked to summarize the local dialogue turns. The doctors were asked to summarize the sections as they would for a typical clinical note by including all the relevant information. Further if the summary included a negated medical term, eg. "doesn't have fever", the doctors were asked to use a [NO] token in front of that particular sentence in the summary. If a local snippet did not contain any relevant information they were excluded from annotations. For example in the beginning or end of conversations there may be turns that are purely greetings and not part of the patient history taking process.

The total dataset contains 1690 number of local snippets with 1365 used for the training set 158 as a validation set and 167 as a held out test set. The test set completely new conversations that were taken from a different date range on the platform compared to the training or validation sets. This was done to ensure that different local snippets from a certain conversation weren't part of the training and test sets. The data was preprocessed by removing the names of the actors in the dialogue ("Doctor", "Patient") and concatenating all the turns within a snippet together.

Since obtaining a larger labelled dataset is expensive and impractical we use the CNN-Daily mail corpus as a pretraining corpus prior to finetuning on our data.




\section{Results}

All the models use a vocabulary size of 50k with 128 dimensional embeddings and 256 dimensional hidden states. The training parameters followed \cite{pointergen} with a learning rate of 0.15 and Adagrad as the optimizer. The coverage mechanism as described in \cite{pointergen} was used for all our models. Models were first pretrained on the CNN-Daily Mail corpus and finetuned on conversational data from our in-house chat-based telehealth platform. All models were finetuned for 8 epochs which was correlated to the lowest validation loss.

The key hyperparameters introduced are the weighting factors used on the additional loss terms (refer sections \ref{subsec:concept}, \ref{subsec:negation} and \ref{subsec:pgen}).
%The hyperparameters were chosen to keep the loss terms within similar orders of magnitude.
$\lambda_m$, $\lambda_n$ and $\delta$ which were used to weight the concept, negation and $p_{\text{gen}}$ loss were set at 1.0, 0.1 and 1.0 to scale the contribution of those terms to be roughly within the same range. For experiments with the 3 mixture model, $\gamma$ the weight on the L1 loss term used to supervise $p_{\text{neg}}$ was set at 2.0. While the $p_{\text{neg}}$ supervision reduced the contributions of the other loss terms we found scaling up the other weights didn't have a material impact on the quantitative and qualitative performance. For simplicity we retained the same hyperparameters for all the models and runs. The bounds for each hyperparameter can be varied within an order of magnitude without significantly impacting the qualitative or quantitative metrics.

Pretraining took approximately 2 days on a single NVIDIA Titan Xp GPU and finetuning took under 2 hours. The concept and negation attention modifications added 512 parameters each to the base pointer generator model with coverage.

\newcommand{\baseline}{2M-BASE~}
\newcommand{\threem}{3M~}
\newcommand{\twompgen}{2M-PGEN~}
\newcommand{\twompgennegation}{2M-PGEN-NEG~}
\newcommand{\threemnegation}{3M-NEG~}
\newcommand{\threempgennegationconcept}{3M-PGEN-NEG-CONCEPT~}

We adopt the following terminology for our models. All of them are pretrained on CNN-DailyMail summarization task.
\begin{itemize}
    \item \textbf{\baseline}: Pretrained pointer generator model fine-tuned on medical dialogue summarization
    \item \textbf{\twompgen}: Pretrained pointer generator model fine-tuned on medical dialogue summarization with the loss described in \ref{subsec:pgen} to control generation probability
    \item \textbf{\twompgennegation}: Pretrained pointer generator model fine-tuned on medical dialogue summarization with the loss described in \ref{subsec:pgen} to control generation probability and the one in \ref{subsec:negation} to improve performance on concept negations

    \item \textbf{\threem}: Pretrained pointer generator model fine-tuned on medical dialogue summarization with explicit negation supervision described in \ref{subsec:negation} without the attention guidance to improve medical concept coverage and negation handling.
    
    \item \textbf{\threempgennegationconcept}: Pretrained pointer generator model fine-tuned on medical dialogue summarization with explicit negation supervision described in \ref{subsec:negation} and the losses described in \ref{subsec:pgen} to control generation probability, \ref{subsec:negation} to improve performance on concept negations and \ref{subsec:concept} to improve medical concept coverage.
\end{itemize}

\subsection{Main Results}


\begin{table*}[ht!]
\begin{tabular}{m{12.5em}|m{1.5cm}|m{1.5cm}|m{1.5cm}|m{1.2cm}|m{1.2cm}|m{1.1cm}|m{0.9cm}}
\hline
\multirow{2}{*}{Models} & \multicolumn{3}{c|}{Metrics} & \multicolumn{4}{c}{Human Evaluation}\\
\cline{2-8}
 & Negation F1 & Concept F1 & ROUGE-L F1 & Model & Baseline & Both & None  \\
\hline
\baseline & $70.1  \pm  0.8$ & $69.1  \pm  1.3$ & $52.6 \pm 0.9$ &- & - & -   & - \\
\hline
\twompgen & $67.3 \pm 3.3$ & $72.8 \pm 0.8$ & $55.4 \pm 0.9$ & 37.1\% & 18.5 \%  & 38.9 \% & 5.3\%\\
\hline
\twompgennegation & $72.2 \pm 3.6$  & $70.9 \pm 2.2$ & $53.5 \pm 0.7$ & 37.7\% & 22.7\% & 34.1\% & 5.4\%\\
\hline
\threempgennegationconcept & $78.0 \pm 4.2$ & $70.6 \pm 1.4$ & $55.2 \pm 1.2$  & 26.9\% & 25.7\%  & 42.5\% & 4.2\%  \\
\end{tabular}
\caption{Automated and Human evaluation.}
\label{tab:learnedlr}

\end{table*}

\input{sections/pgen_modulation}

We evaluated the different models considering the following three properties that we identified to be important in medical dialogue summarization.

\TODO{this needs to align with metrics}

1. Bias towards copying text from the snippet.

2. Covering all medical concepts from the snippet.

3. Preserving the correct negation / affirmation of medical conditions i.e. if a user has / doesn't have a symptom X, the summary should correctly reflect that. 

Table 1. describes the key findings from our work. We observe that on automated metrics different models perform best on different tasks such as negation correctness and concept coverage. Explicit negation modeling like negation attention and 3-mixture modeling boost performance on negatives \TODO{If we name these metrics, we can use consistent terminology throughout} while utilizing a $p_{\text{gen}}$ loss boosts concept performance. Multiple studies in dialogue and conversational AI have shown that automated metrics don't necessarily correlate well with human evaluation \cite{fair, meena, salesforcemetrics}. Given that these summaries would be used as clinical notes by doctors, we had the model outputs annotated by two doctors to determine overall quality. Doctors preferred \twompgen over \baseline~more than any other model. On a head to head comparison between each model and \baseline, \twompgen is preferred on 37\% of the  examples while \baseline is preferred on 18\% of the examples. This difference is the highest among all models compared. On observing the outputs, models with the $p_{\text{gen}}$ loss were more coherent and copied much of the original phrasing in the dialogue which was preferred by the doctors.

Further on the human evaluation task where the model's output summary was graded on whether it included ``all'', ``most'', ``some'', ``none'' of the relevant information, \twompgen gets all or most of the information on 80\% of examples compared to 60\% for \baseline.

\begin{figure}
\label{fig:task1}
    \centering
    \includegraphics[height=5cm,width=8cm]{sections/figures/Task1.png}
    \caption{Human Evaluation of amount of relevant information covered by summaries}
    
\end{figure}
\input{sections/3mixturecomparison}

\subsection{Role of explicitly modulating $p_{\text{gen}}$}

One reason why explicitly modulating $p_{\text{gen}}$ produces strong human evaluation outcomes is that summarizing dialogue involves guiding the copy mechanism to shift attention distributions over to patient answers and back to doctor questions as opposed to linear copying. Without explicit signal, the model learns the easier mechanism of using the copy mechanism sparingly while relying on the generator to build the summary. By penalizing $p_{\text{gen}}$ the model has to make the trade-off between using the generator and improving cross entropy loss. It can only reduce the overall loss using the generator distribution if the reduction in cross entropy loss compensates for the $p_{\text{gen}}$ penalty.

From Table~\ref{fig:pgen} we observe that \baseline relies more on the generator to create the summaries and at times doesn't copy from the patient's answers. In the second example, "no" is copied from the patient \twompgen while "no" is produced by the generator in \baseline indicating its inability to copy between actors in the dialogue.


\subsection{Role of encoding medical concepts}

Given data sparsity our hypothesis was that directly using medical concepts to guide the attention mechanism would help performance on the concept metric. We do see improvement in this metric when adding concept attention to \baseline (concept F1 72.0 vs 69.1) however once $p_{gen}$ loss is introduced we notice these gains no longer hold. On local snippets, we observe that the increased copying ability compensates for the removal of concept attention and adding concept attention causes a loss in performance. In both cases the attention on medical concepts in the copy distribution increases 5\% however this doesn't amount to consistent increase on the automated metrics. We leave this as an open research direction for longer dialogue snippets where enhanced copying may need to be couple with concept attention.


\subsection{Role of explicit negation modeling} 
To improve on the negation performance we evaluated 3-mixture models that incorporate negations explicitly in the attention mechanism as well as a third mixture $p_{\text{neg}}$ in the final probability distribution as described in \ref{subsec:negation}. From Table~\ref{tab:learnedlr}, we observe that \twompgennegation improves Negation F1 over \twompgen (72.2 vs 67.3) and introducing 3 mixture modeling helps boost Negation F1 further. 

From Table \ref{tab:quant3m} we see that a vanilla 3M model without enhancements to the attention improves on negations over \baseline and further improvement is seen when using the negation attention and associated loss term.


% Since $p_{\text{neg}}$ controls the generation of [NO] and [NO] is sparsely prevalent in the reference, the ideal distribution of $p_{\text{neg}}$ over the length of decoding is to hit 1.0 during [NO] generation and 0 elsewhere. Supervising $p_{\text{neg}}$ explicitly with an L1 loss to maximise the margin between $p_{\text{gen}}$ + $p_{\text{copy}}$ and $p_{\text{neg}}$ helps enforce the model to learn this distribution of $p_{\text{neg}}$.

\begin{table}[ht!]
\begin{tabular}{m{2cm}|m{1.5cm}|m{2cm}}
\hline
Model & Negation F1 & ROUGE-L F1   \\
\hline
\baseline & $70.1  \pm  0.8$
& $52.6 \pm 0.9$  \\
\hline
\threem   & $76.9 \pm 3.6$ & $56.4 \pm 0.3$ \\
\hline
\threemnegation & 81.5 & 54.5 \\
\hline

\end{tabular}
\caption{Negation Ablation both as a switching variable and word attention}
\label{tab:quant3m}

\end{table}













==> sections/extra.tex <==
Model & Negation F1 & Affirmative F1 & Coverage F1 & ROUGE-1 F1 & ROUGE-L F1\\
2 mixture + concept & 0.71 & 0.89 &	0.72 &	0.57 & 0.53\\
3 mixture baseline  & 0.82	& 0.92	& 0.7 & 0.58 & 0.55\\
3 mixture + concept attention & \textbf{0.83} & \textbf{0.93} & 0.69 & \textbf{0.59} & 0.54\\
3 mixture + gen loss & 0.73	& 0.89	& 0.7	& 0.6	& \textbf{0.56}\\



\begin{table*}[ht!]


\begin{tabular}{p{0.2\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}}
\hline
Model & Negation F1 & Affirmative F1 & Coverage F1 & ROUGE-1 F1 & ROUGE-L F1\\
\hline
2 mixture baseline & 0.70 & 0.87 & 0.69 & 0.57 & 0.53\\
2 mixture + gen loss & 0.66 & 0.89 & 0.73 & 0.58 & 0.55\\
2 mixture + negation + gen loss & 0.72 & \textbf{0.90} & 0.71 & 0.58 & 0.55\\
2 mixture + negation + concept + gen loss & 0.66 & 0.87 & \textbf{0.74} & 0.59 & 0.55\\
3 mixture + concept attention + gen loss & \textbf{0.80} & \textbf{0.90} & 0.68 & 0.51 & 0.53\\
\hline

\end{tabular}
\caption{Comprehensive model performance on automated metrics.}
\end{table*}

==> sections/figures_old.tex <==

\begin{figure}{\columnwidth}
\caption{Modulating $p_{gen}$: Pink is used to show words copied from the Doctor, green for words copied from the Patient and orange for words generated.}
\label{fig:pgen}
\begin{tabular}{ |p{7cm}| } 
\hline
1. DOCTOR : Thanks for letting me know. How severe is the pain on a scale of 1-10, considering 10 being the worst and severe? 
 
PATIENT: 4-5\\

\hline
\textbf{2 mixture + $p_{gen}$ loss}

\colorbox{pink}{the pain is} \colorbox{green}{4-5} \colorbox{pink} {on a scale} \colorbox{pink}{of 1} \colorbox{orange}{-} \colorbox{pink}{10 being the worst and severe}\\
\hline

\textbf{2 mixture baseline}

\colorbox{pink}{pain} \colorbox{orange}{is} \colorbox{pink} {severe} \colorbox{orange}{.} \colorbox{pink}{pain} \colorbox{orange}{is} \colorbox{pink}{10} \colorbox{orange}{on} \colorbox{pink}{a scale} \colorbox{orange} {of 1-10.}\\


\hline
\\
2. DOCTOR: does your chest pain get worse while taking deep breaths ?

PATIENT: no \\

\hline

\textbf{2 mixture + $p_{gen}$ loss}

\colorbox{green}{no} \colorbox{pink}{chest pain} \colorbox{orange}{get} \colorbox{pink}{worse} \colorbox{pink}{while taking deep breaths} \\

\hline

\textbf{2 mixture baseline}

\colorbox{orange}{no} \colorbox{pink}{chest pain} \colorbox{orange}{. worse} \colorbox{pink}{while} \colorbox{pink}{taking breaths}\\
\\
\hline
\\
3. DOCTOR: Thanks for sharing. Have you been on any medications for the same?

PATIENT: I’ve been on isotretenoin for the acne but off of it for the last 5 months nothing for the bradycardia\\


\hline
\textbf{2 mixture + $p_{gen}$ loss}

\colorbox{green}{been on isotretenoin for the acne} \colorbox{green}{but off of it for the last 5 months}\\

\hline
\textbf{2 mixture baseline}

\colorbox{orange}{not} \colorbox{green}{on isotretenoin for acne} \colorbox{orange}{but} \colorbox{green}{off of bradycardia for last 5 months} \colorbox{orange}{.}\\
\hline




\end{tabular}

\end{figure}



\begin{table}[ht!]
\begin{tabular}{|m{7cm}|}
\hline
1. DOCTOR: do you have chest pain while coughing?

PATIENT: yes and breathing. pretty much all the time \\
\hline
3 Mixture Model: \textbf{\textcolor{blue}{has chest pain}} while coughing a and breathing.  \\
\\

2 Mixture Model: \textbf{\textcolor{red}{no chest pain}} while coughing. pretty much all time.\\
\hline
\\
2. DOCTOR: did you take any medication for it?

PATIENT: no\\
\hline
3 Mixture Model: \textbf{\textcolor{blue}{[NO] not taking any medication}} for it\\
\\
2 Mixture Model: \textbf{\textcolor{red}{took medication}} for it.\\
\hline
\end{tabular}
\caption{Improvements on Negatives and Affirmatives with 3 mixture model}
\label{tab:qual3m}

\end{table}

==> sections/model.old.tex <==
\section{Modeling}



\subsection{Pointer Generator Network}

The Pointer Generator architecture proposed by See et al. allows for hybrid abstractive and extractive summarization. The model is an extension of the sequence to sequence architecture with attention and allows for copying of words from the source text using a pointer mechanism and generation of words from a fixed vocabulary using the decoder probability distribution at every time step of decoding. $p_{gen}$ is computed as a soft switch between the copying and generation distributions. A final probability distribution is obtained as follows for each decoding step.
\[P(w) = p_{gen} * P_{vocab} + (1-p_{gen}) * \sum_{i}a^t_i \]
This vocabulary distribution is on the union of the words that appear in the source and the fixed vocabulary allowing the model to copy out of vocabulary words.

See et al. observe that while the Pointer Generator Network ends training with $p_{gen}$ at 0.53 during inference, $p_{gen}$ is far lower (0.17). This implies that the model has higher tendency for extractive summarization and copying from the source. 

These inductive biases described are desirable for the task of medical dialogue summerization. The summary produced at the end of the dialogue should have majority of the text copied to preserve the integrity of the symptoms and medical issues discussed. At the same time, it is important to handle out of vocabulary terms used by patients and doctors that may describe particular medical conditions and terms. 

However from Figure 2 it's clear that a pointer generator network trained on news corpora learns to copy text in a sequential fashion. This method of summarization is perfectly valid for news articles however for dialogue, a model would be required to go back and forth between the doctor questions and patient answers to copy the complete summary. This shifting of copy distributions back and forth in the source snippet isn't learnt by a baseline Pointer Generator trained on CNN-Daily Mail.

\subsection{Medical Concept Attention}

In medical dialogue summarization it is important to include medical conditions and terms used during the dialogue in the summary. Given millions of pairwise dialogues and summaries it may be possible to learn to pay attention to medical terms without explicit modeling however given smaller datasets, we propose to model this domain knowledge explicitly.

Given a knowledge base of known medical concepts we propose creating encodings of concepts that occur in the source snippet that are also present in the reference. Since the intention is to influence the attention distrbution to focus on medical terms, these encodings are used as part of the summation to compute the attention distribution. 


\[e^t_i = v^t tanh(W_h*h_i + W_s*s_t + w_c*c^t_i \]
\[+ w_a*{kb}_i^t + b_{attn})\]

\[a^t = softmax(e^t)\]
where $h_i$ is the encoder hidden state, $s_t$ is the decoder hidden state, $c_t$ is the coverage vector described in See et al. and $kb$ is a one-hot encoded vector of presence of concepts in the source snippet with the same dimension as the source snippet.

Analogous to the coverage mechanism introduced by See et al. we propose to model this both from the attention mechanism as well as the loss function to directly supervise the model.

The full loss function is formulated as such.

\[{loss}_t = -\log{P(w^*_t)} + \lambda * \sum_{i} min(a^t_i,c^t_i) b\]
\[+ k*(1 - \sum_{i}ca^t_i)\] 

Where the additional term used to supervise the concept attention is
\[k*(1 - \sum_{i}ca^t_i)\] where k is a scalar factor on the concept loss term and $ca$ is the dot product between $kb$ and $a^t$. This term encourages higher attention weights on positions where concepts are present.

Since the concepts are encoded based on whether it's present in the reference this acts as a form of teacher forcing where the concepts are encoded and supervised only during training time but at test time, these encodings are not provided to the model. It's important to only encode concepts that are in the reference to prevent extraneous words and phrases from appearing in the decoded summary.

\subsection{Negation Attention}

Another critical component in medical dialogue summarization is getting the negations on medical concepts and symptoms correct. Again, this could be learnt implicitly given enough training data but given smaller datasets, we propose to model this explicitly.

We propose modeling this similarly to how we model concept information by influencing the attention mechanism and directly supervising the model in the loss function. We propose encoding all the negative terms (no, nope, not etc.) in the source snippet to provide explicit information to the model to focus the attention distribution on those words.
\[e^t_i = v^t tanh(W_h*h_i + W_s*s_t + w_c*c^t_i \]
\[+ w_a*{kb}_i^t + w_n*{n}_i^t + b_{attn})\]where $n$ is the one-hot encoded negation words in the source snippet.

Similar to concept attention loss, we use an additional term called the negation attention loss \[k*(1 - \sum_{i}na^t_i)\] where $na$ is the dot product between the negation encoding and the attention mechanism to promote higher weights on negation words.

\subsection{3 Mixture Model}

(Need better way to phrase this )Based on the experimental evidence, it was clear that a more aggressive method of modeling negations was needed.

We propose providing explicit negation labels in the labeled summaries by including a [NO] prior to occurrence of negated concepts. The [NO] token was also added to the fixed vocabulary. The model would need to learn when to generate the [NO] token in the final decoded summary. However leveraging $p_{gen}$ to generate [NO] would influence the likelihood of $p_{gen}$ in other abstractive parts of the summary and from our experiments we observed that it reduced coherence by inflating $p_{gen}$. We propose to separate the generation of [NO] from the copy and generation mechanism. We formulate the final probability distribution as a combination of three terms $p_{gen}$, $p_{copy}$, $p_{neg}$ where $p_{neg}$ controls the generation of [NO]. In this formulation, probability mass on $p_{neg}$ will be drawn from $p_{copy}$ and $p_{gen}$ and not just $p_{gen}$.

We propose the final probability distribution on each decoding time step as follows.
\[P(w) = p_{gen} * P_{vocab} + p_{copy} * \sum_{i}a^t_i + p_{neg}*P_{[NO]}\]

\[p_{gen}, p_{copy}, p_{neg} = softmax(w^T_{h^*}h^*_t + w^T_{s}s_t\]
\[+ w^T_{x}x_t + b_{ptr})\]

To guide the model we propose to explicitly supervise $p_{neg}$. The labels used for supervision would be the groundtruth for $p_{neg}$ which is 1 at positions with [NO] and 0 elsewhere. In positions where $p_{neg}$ is 0, $p_{gen} + p_{copy}$ would be 1. The loss function used to supervise $p_{neg}$ is L1 and not a classification loss like cross entropy because the margin of separation of the probabilities is more crucial than getting the class correct. [NO] occurs sparsely in the reference text and when it's present, the model needs to have high probability mass on $p_{neg}$ so that the final probability distribution is dominated by $p_{neg}$. Since the desired behavior of $p_{neg}$ is to sparsely spike, it's not sufficient for $p_{neg}$ to be marginally higher than $p_{copy}$ and $p_{gen}$ which is what cross entropy loss would encourage. Instead the difference between $p_{neg}$ and $p_{gen} + p_{copy}$ needs to be as large as possible.

\subsection{Patient Attention}


==> sections/model2.tex <==
\section{Model}

\begin{figure}{\columnwidth}
\caption{Vanilla Pointer Generator learns to produce sequential copying outputs as opposed to the back and forth needed for dialogue}
\label{fig:pgen}
\begin{tabular}{ |p{7cm}| } 
\hline
\textbf{Excerpt CNN-Daily Mail}

\textcolor{blue}{porto boss julen lopetegui}(left) \textcolor{blue}{was hugged by fans congratulating him on their champions league run.} police escorts were needed to keep the delirious supporters at bay as the porto from porto supporters team bus drove past.
\\

\hline
\textbf{Pointer Generator}

\textcolor{blue}{porto boss julen lopetegui was hugged by fans congratulating him on their champions league run.}
\\

\hline
\\
DOCTOR : Thanks for letting me know. How severe is the \textcolor{blue}{pain on a scale of 1-10}, considering \textcolor{blue}{10 being the worst and severe? }
 
PATIENT: \textcolor{orange}{4-5}\\

\hline

\textbf{Reference}

\textcolor{blue}{pain} is \textcolor{orange}{4-5}/10 \textcolor{blue}{on a scale of 1-10} with \textcolor{blue}{10 being worse and severe.} \\

\hline



\end{tabular}

\end{figure}


Extractive summarization of news articles usually needs ``sequential'' copying i.e. parts of the article that need to be copied appear sequentially without having to be revisited. Therefore, this is what a pointer generator network \cite{pointergen} trained on news corpora such as CNN-Daily Mail \TODO{cite cnn-daily-mail} would learn. While perfectly valid for news articles, figure~\ref{fig:pgen} illustrates how medical dialogue summarization requires the model to go back and forth between the doctor questions and patient answers to copy the complete summary. While the pointer generator network can handle this by switching between generation and copying, we explicitly want summaries to be copied as much as possible from the source dialogue since factual errors  in a medical setting are unacceptable. This need to shift copy distributions back and forth between doctor and patient turns in the source snippet cannot be easily learned by a pointer generator network trained on CNN-Daily Mail.

\subsection{Base model: Pointer Generator Network}

The pointer generator architecture proposed by allows for hybrid abstractive and extractive summarization. The model is an extension of the sequence to sequence architecture with attention and allows for copying of words from the source text using a pointer mechanism and generation of words from a fixed vocabulary using the decoder probability distribution at every time step of decoding. $p_{gen}$ is computed as a soft switch between the copying and generation distributions. At each decoding step, a final probability distribution $P(w)$ over the extended vocabulary is obtained as follows

\[P(w) = p_{\text{gen}} P_{\text{vocab}}(w) + (1-p_{\text{gen}}) \sum_{i:w_i=w}a^t_i \]
where $P_{\text{vocab}}$ is a probability distribution over all words in the vocabulary and $a^t$ is the attention distribution i.e.  a probability distribution over the source words that tells the decoder where to look to produce the next word. This vocabulary distribution is on the union of the words that appear in the source and the fixed vocabulary allowing the model to copy out of vocabulary words.

\cite{pointergen} observe that while the pointer generator network ends training with $p_{gen}$ at 0.53, $p_{gen}$ is far lower (0.17) at inference. This implies that the model has higher tendency for extractive summarization and copying from the source. This inductive bias described is desirable for the task of medical dialogue summarization. The summary produced at the end of the dialogue should have majority of the text copied to preserve the integrity of the symptoms and medical issues discussed. At the same time, it is important to handle out of vocabulary terms used by patients and doctors that may describe particular medical conditions and terms.

\subsection{Incorporating medical knowledge}
%\subsection{Medical Concept Attention}

In medical dialogue summarization it is important to include medical conditions and terms used during the dialogue in the summary. We highlight some such terms in the example in figure~\ref{fig:example} \TODO{refer to examples introduced in the intro -- if we sufficiently describe need
for incorporating kb in intro, we can skip `why' here}. Given millions of pairwise dialogues and summaries it may be possible to learn to pay attention to medical terms without explicit modeling however given smaller datasets, we propose to model this domain knowledge explicitly.

Given a knowledge base of known medical concepts we propose creating encodings of concepts that occur in the source snippet that are also present in the reference. Since the intention is to influence the attention distrbution to focus on medical terms, these encodings are used as part of the summation to compute the attention distribution. 

\[ e^t_i = v^t~\text{tanh}(W_hh_i + W_ss_t + w_cc^t_i + w_m{m}_i^t + b_{\text{attn}}) \]
\[ a^t = \text{softmax}(e^t) \]
where $h_i$ is the encoder hidden state, $s_t$ is the decoder hidden state, $c_t$ is the coverage vector described in \cite{pointergen} and $m^t$ is a one-hot encoded vector of presence of medical concepts in the source snippet with the same dimension as the source snippet.

Analogous to the coverage mechanism introduced by \cite{pointergen}, we propose to model this both, in the attention mechanism as well as in the loss function to directly supervise the model.

The full loss function is formulated as such.

\begin{equation*}
\begin{split}
{\text{loss}}_t= &-\log{P(w^*_t)} + \lambda\sum_{i} \text{min}(a^t_i,c^t_i)~b \\ & + k(1 - \sum_{i}{m_{\text{attn}}}^t_i)
\end{split}
\end{equation*}

where k is a scalar factor on the concept loss term and ${m_{\text{attn}}}^t$ is the dot product between $m^t$ and $a^t$. This term encourages higher attention weights on positions where concepts are present.

Since the concepts are encoded based on whether they are present in the reference, this acts as a form of teacher forcing where the concepts are encoded and supervised during training time but at test time, these encodings are not available to the model. It is important to only encode concepts that are in the reference to prevent extraneous words and phrases from appearing in the decoded summary. \TODO{needs more clarity}

\subsection{Modeling negations }

Another critical component in medical dialogue summarization is to negate medical concepts and symptoms correctly, as described in the source dialogue. \TODO{refer to examples introduced in the intro -- if we sufficiently describe need
for negation modeling in intro, we can skip `why' here} While this could be learnt implicitly given enough training data, we propose to model this explicitly for a low-data scenario.

We propose modeling negations in two ways
\begin{itemize}
    \item Attention mechanism on negation words
    \item Explicit switching variable that is sampled, inducing a mixture model over copy, generate and negate
\end{itemize}

\noindent {\bf Negation word attention:}  We propose modeling this the same way we model medical concept information by influencing the attention mechanism and directly supervising the model in the loss function. We propose encoding all the negative terms such as `no', `nope', `not' etc. in the source snippet to provide explicit signal to the model to focus the attention distribution on such terms.

\begin{equation*}
\begin{split}
e^t_i ={} v^t~\text{tanh}(&W_hh_i + W_ss_t + w_cc^t_i +{} \\ &w_m{m}_i^t + w_n{n}_i^t + b_{\text{attn}})
\end{split}
\end{equation*}

Similar to concept attention loss, we use an additional term called the negation attention loss \[k(1 - \sum_{i}{n_{\text{attn}}}^t_i)\] where ${n_{\text{attn}}}$ is the dot product between the negation encoding and the attention mechanism to promote higher weights on negation words.


%(Need better way to phrase this )Based on the experimental evidence, it was clear that a more aggressive method of modeling negations was needed.
\noindent {\bf Negation as a switching variable:}
%\TODO{Explain rationale for this, in addition to negation attention} 
Our labeled data contains explicit negation labels in the reference summaries as a `[NO]' token prior to occurrence of negated concepts (see figure~\ref{fig:example}. This was provided as a labeling instruction to the labelers.

While the [NO] token can be added to the fixed vocabulary, we note that the model would need to learn when to generate the [NO] token in the final summary using the decoder. However leveraging $p_{\text{gen}}$ to generate [NO] would influence the likelihood of $p_{\text{gen}}$ in other abstractive parts of the summary. From our experiments we also observed that it reduced coherence by inflating $p_{\text{gen}}$. We, therefore, propose to separate the generation of [NO] from the copy and generation mechanism. We formulate the final probability distribution as a combination of three terms $p_{\text{gen}}$,~$p_{\text{copy}}$,~$p_{\text{neg}}$ where $p_{\text{neg}}$ controls the generation of [NO]. In this formulation, probability mass on $p_{\text{neg}}$ will be drawn from $p_{\text{copy}}$ and $p_{\text{gen}}$ and not just $p_{\text{gen}}$.

We propose the final probability distribution on each decoding time step as follows.
\begin{equation*}
\begin{split}
    P(w) ={} & p_{\text{gen}}P_{\text{vocab}}(w) + p_{\text{copy}}\sum_{i:w_i=w}a^t_i +{} \\ & p_{\text{neg}}P_{\text{[NO]}}
\end{split}    
\end{equation*}

\begin{equation*}
\begin{split}
p_{\text{gen}},~p_{\text{copy}},~p_{\text{neg}} ={} \text{softmax}(&w^T_{h^*}h^*_t + w^T_{s}s_t +{} & \\ & w^T_{x}x_t + b_{ptr})
\end{split}
\end{equation*}

\TODO{Anirudh please add explanation for the variables above. $w_x$ and $x_t$ aren't defined anywhere}

To guide the model we explicitly supervise $p_{\text{neg}}$. The labels used for supervision would be the ground truth for $p_{\text{neg}}$ which is 1 at positions with a [NO] token in the labeled summary and 0 elsewhere. In positions where $p_{\text{neg}}$ is 0, $p_{gen} + p_{copy}$ would be 1. [NO] occurs sparsely in the reference text and when it is present, the model needs to have high probability mass on $p_{neg}$ so that the final probability distribution is dominated by $p_{\text{neg}}$. Since the desired behavior of $p_{\text{neg}}$ is to peak sparsely, it is not sufficient for $p_{\text{neg}}$ to be marginally higher than $p_{\text{copy}}$ and $p_{\text{gen}}$ which is what a cross entropy loss would encourage. Instead the difference between $p_{neg}$ and $p_{gen} + p_{copy}$ needs to be as large as possible. Therefore, the loss function used to supervise $p_{\text{neg}}$ is L1 and not cross entropy.

\TODO{describe the final multihead loss and attention succinctly}

\subsection{Controlling Generation Probability}

\cite{pointergen} mention that during inference time $p_{\text{gen}}$ is below 0.2. We see that a zero shot pointer generator model trained on CNN-Daily Mail does have a zero-shot average $p_{\text{gen}}$ of 0.2 on our medical dialogue dataset. However after fine-tuning on our dataset, we observe that the average $p_{\text{gen}}$ is 0.4 at inference time. Our hypothesis is that the medical dialogue summarization task is difficult for the copy mechanism to learn given limited data since $p_{\text{copy}}$ has to shift the distribution back and forth between patient answers and parts of the doctor's questions. Rather than learning to constantly shift the copy distribution the model learns to use the generator more. This is detrimental to our task since most of the information for the summary is present in the dialogue and we want the model to be biased to copying directly from the source rather than generate tokens.

We propose a penalty on the model for using the generator distribution instead of the copy distribution to force it to learn to use the copy mechanism effectively. We add $\delta \cdot p_{\text{gen}}$ term to the overall loss where $\delta$ is a scalar constant. This term will be large if the model is using the generator more during decoding.

==> sections/more_examples.tex <==
 %CUSTOMER| the doctor prescribed ventolin when i ’ ve been on proair for years , i would like to be on proair as it is cheaper with my insurance plan 	prescribed ventolin when on proair for years . would like to be on proair as it is cheaper with insurance plan .	was on proair for years and would like to be on proair .	
\begin{table*}[]

\centering
\resizebox{\textwidth}{!}{\begin{tabular}{lll}
\toprule
\hline

\textbf{Snippet}   & \textbf{\baseline} & \textbf{\twompgen} \\ 
\hline


\begin{tabular}[c]{@{}l@{}}
PATIENT: the doctor prescribed ventolin \\ \hspace{.7in} when I’ ve been on proair for years\\
  \hspace{.7in} I would like to be on proair  as\\
  \hspace{.7in} it is cheaper with my insurance plan   \\

\end{tabular}  &

\begin{tabular}[c]{@{}l@{}}
was on proair for years and \\would like to be on proair.
\end{tabular} &
\begin{tabular}[c]{@{}l@{}}
prescribed ventolin when on proair for years.\\
would like to be on proair as it is cheaper \\ with insurance plan.
\end{tabular}  
\\ \hline



\begin{tabular}[c]{@{}l@{}}
DOCTOR: what color is the phlegm ?
 \\
 PATIENT: dark green dark green \\
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}
the color is the phlegm .
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}
the phlegm is dark green dark green\\

\end{tabular}
\\ \hline


\begin{tabular}[c]{@{}l@{}}
DOCTOR: Did you take any medication for it?\\
PATIENT: no
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}
took medication for it.
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}
no taking medication for it.

\end{tabular}
\\ \hline

\end{tabular}}
\caption{More Examples}
\label{fig:moreeg}
\end{table*}




\begin{table*}[]

\centering
\resizebox{\textwidth}{!}{\begin{tabular}{lll}
\toprule
\hline

\textbf{Snippet}   & \textbf{\threempgennegationconcept} & \textbf{\twompgen} \\ 
\hline


\begin{tabular}[c]{@{}l@{}}
DOCTOR: hello sidney , my name is dr. williams. \\ \hspace{.7in} I am happy to assist you with your health \\ \hspace{.7in} concern today. I can see that you injured  \\ \hspace{.7in} your hand, and were already evaluated by another doctor.  \\ \hspace{.7in} The xrays showed no broken bones. \\\hspace{.7in} How can I help you today ? \\

PATIENT: the doctor had said since she didn’t see any fracture \\\hspace{.7in} that it could be a really bad sprain \\\hspace{.7in} she did tell me to wait 7 days.

\end{tabular}  &

\begin{tabular}[c]{@{}l@{}}
\text{[NO]} no broken bones by another doctor .\\ the xrays showed no broken fracture
\end{tabular} &
\begin{tabular}[c]{@{}l@{}}
no injured hand , were evaluated by another doctor .\\ xrays showed no broken bones .
\end{tabular}  
\\ \hline



\begin{tabular}[c]{@{}l@{}}
DOCTOR: For a while as in few weeks or months?\\

PATIENT: I noticed it maybe a month ago I don't look \\ \hspace{.7in} at my chest that often because I've got \\ \hspace{.7in} a lot of dysphoria so I'm not really sure\\\hspace{.7in} how long it's been there
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}
has been there for a month ago . \\
\text{[NO]} not sure how long the lot of dysphoria .
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}
noticed it maybe a month ago. \\don't look at chest that often because 've got a lot of dysphoria.\\ not sure how long it's been there in months.\\

\end{tabular}
\\ \hline

\end{tabular}}
\caption{More Examples}
\label{fig:moreeg2}
\end{table*}
